From Dissonance to Insights: Dissecting Disagreements in Rationale Construction for Case Outcome Classification

In legal NLP, Case Outcome Classification (COC) must not only be accurate but also trustworthy and explainable. Existing work in explainable COC has been limited to annotations by a single expert. However, it is well-known that lawyers may disagree in their assessment of case facts. We hence collect a novel dataset RAVE: Rationale Variation in ECHR1, which is obtained from two experts in the domain of international human rights law, for whom we observe weak agreement. We study their disagreements and build a two-level task-independent taxonomy, supplemented with COC-specific subcategories. To our knowledge, this is the first work in the legal NLP that focuses on human label variation. We quantitatively assess different taxonomy categories and find that disagreements mainly stem from underspecification of the legal context, which poses challenges given the typically limited granularity and noise in COC metadata. We further assess the explainablility of SOTA COC models on RAVE and observe limited agreement between models and experts. Overall, our case study reveals hitherto underappreciated complexities in creating benchmark datasets in legal NLP that revolve around identifying aspects of a case's facts supposedly relevant to its outcome.

==> table/RQ2.tex <==

\begin{table*}[]
\caption{Agreement and prediction scores of RQ2, RQ3 methods.
standard error of Kappa score in parentheses; alignment is measured over the same 40 cases; prediction performance is measured over respective test sets mentioned in each RQ section.
}
\scalebox{0.8}{
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
Variants   &   Base model            & Kappa A1                   & Kappa A2                   & micF1              & macF1              & hm-F1         \\ \hline
\multirow{3}{*}{facts+law with aux. task} & BERT                  & 11.74 (3.75)               & 9.11 (3.36)                & 56.23                 & 59.79                 & 55.57                 \\ \cline{2-7} 
                                                               & LegalBERT             & 11.67 (3.63)               & 9.03 (2.81)                & 57.13                 & 60.38                 & 58.19                 \\ \cline{2-7} 
                                                             & CaselawBERT               & 11.73 (3.73)               & 9.22 (3.14)                & 57.47                 & 59.94                 & 56.65                 \\ \cline{1-7} 
\multirow{3}{*}{facts with  aux. task}     & BERT                  & 11.63 (2.94)               & 9.27 (3.61)                & 57.46                 & 59.68                 & 56.08                 \\ \cline{2-7} 
                                                            & LegalBERT             & 11.58 (3.15)               & 9.13 (3.23)                & 58.46                 & 60.89                 & 57.44                 \\ \cline{2-7} 
                                                           & CaselawBERT               & 11.69 (3.28)               & 9.41 (3.51)                & 57.94                 & 59.68                 & 56.59                 \\ \hline
\multirow{3}{*}{facts+law with no aux. task} & BERT                  & 11.39 (3.32)               & 8.97 (3.81)                & 54.36                 & 57.86                 & 55.22                 \\ \cline{2-7} 
               & LegalBERT             & 11.17 (3.15)               & 8.72 (3.17)                & 53.23                 & 57.19                 & 55.07                 \\ \cline{2-7} 
                                                  & CaselawBERT               & 11.62 (3.43)               & 8.83 (3.29)                & 54.12                 & 57.72                 & 55.35                 \\ \cline{1-7} 
\multirow{3}{*}{facts with no aux. task}    & BERT                  & 11.12 (3.44)               & 9.02 (3.62)                & 53.52                 & 57.22                 & 55.2                  \\ \cline{2-7} 
                      & LegalBERT             & 11.02 (3.66)               & 8.88 (3.62)                & 53.71                 & 58.04                 & 55.58                 \\ \cline{2-7} 
                        & CaselawBERT               & 11.16 (3.38)               & 8.93 (3.28)                & 53.63                 & 57.14                 & 55.34                 \\ \hline
\multicolumn{2}{|c|}{Hard Match}   &   \multicolumn{1}{r|}{19.76} & \multicolumn{1}{r|}{16.59} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} \\ \hline
\multicolumn{2}{|c|}{Random baseline}   &   \multicolumn{1}{r|}{7.62} & \multicolumn{1}{r|}{5.81} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} \\ \hline \hline
\multicolumn{1}{|l|}
{\multirow{3}{*}{Fact classification}}
& \multicolumn{1}{l|}{BERT}      & \multicolumn{1}{l|}{11.48 (3.62)} & \multicolumn{1}{l|}{9.22 (3.29)} & \multicolumn{1}{c|}{65.52}    & \multicolumn{1}{c|}{74.97}    & \multicolumn{1}{c|}{57.97}      \\ \cline{2-7}
\multicolumn{1}{|l|}{}                                     & \multicolumn{1}{l|}{LegalBERT} & \multicolumn{1}{l|}{11.37 (3.66)} & \multicolumn{1}{l|}{9.18 (2.94)} & \multicolumn{1}{c|}{66.03}    & \multicolumn{1}{c|}{76.49}    & \multicolumn{1}{c|}{58.42}       \\ \cline{2-7}
\multicolumn{1}{|l|}{}                                     & \multicolumn{1}{l|}{CaselawBERT}   & \multicolumn{1}{l|}{11.59 (3.71)} & \multicolumn{1}{l|}{9.37 (3.58)} & \multicolumn{1}{c|}{65.84}    & \multicolumn{1}{c|}{75.35}    & \multicolumn{1}{c|}{58.17}       \\ \cline{1-7}
\multirow{3}{*}{Article aware Prediction} & \multicolumn{1}{l|}{BERT}      & \multicolumn{1}{l|}{11.75 (3.64)} & \multicolumn{1}{l|}{9.57 (3.44)} & \multicolumn{1}{c|}{74.43}    & \multicolumn{1}{c|}{80.35}    & \multicolumn{1}{c|}{61.22}\\ \cline{2-7}
\multicolumn{1}{|l|}{}                                     & \multicolumn{1}{l|}{LegalBERT} & \multicolumn{1}{l|}{11.53 (3.51)} & \multicolumn{1}{l|}{9.31 (3.53)} & \multicolumn{1}{c|}{74.58}    & \multicolumn{1}{c|}{80.83}    & \multicolumn{1}{c|}{61.35}          \\ \cline{2-7}
\multicolumn{1}{|l|}{}                                     & \multicolumn{1}{l|}{CaselawBERT}   & \multicolumn{1}{l|}{11.82 (3.66)} & \multicolumn{1}{l|}{9.79 (3.22)} & \multicolumn{1}{c|}{74.49}    & \multicolumn{1}{c|}{80.95}    & \multicolumn{1}{c|}{61.38}         \\ \cline{1-7}
\end{tabular}}

 \label{tab:rq2}
\end{table*}

==> table/iaa.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]

 \caption{Inter-Annotator Agreement Statistics. `Metadata' indicates whether this allegation is in the HUDOC metadata. Kappa scores less than the 25th percentile (0.12) are highlighted. Value in brackets indicates standard error.}
\scalebox{0.8}{

\begin{tabular}{|c|c|c|c|}
\cline{1-4}
\textbf{Alleged}                        & \textbf{Metadata}                       & Kappa V                               & Kappa $\lnot$ V  \\ \cline{1-4}
\textbf{14}                                     &                                         & &  \cellcolor[HTML]{D9D9D9}13.70 (3.81)  \\ \cline{1-1}
\textbf{2}                                      &                                         & & \cellcolor[HTML]{D9D9D9}00.00 (0.00)  \\ \cline{1-1}
\textbf{3}                                      &                                         & & \cellcolor[HTML]{D9D9D9}11.33 (0.00)  \\ \cline{1-1}
\textbf{6}                                      &                                         & & \cellcolor[HTML]{D9D9D9}7.05 (15.26)  \\\cline{1-1}
\textbf{8}                                      &                                         & & 18.54 (14.24)                         \\\cline{1-1}
\textbf{P1-1}                                   & \multirow{-6}{*}{\textbf{0}}            & & \cellcolor[HTML]{D9D9D9}00.00 (00.00) \\ \cline{1-4}
\textbf{10}                   &                                         & 27.84 (8.82)                          & 36.27 (4.21) \\ \cline{1-1}
\textbf{11}                   &                                         & 25.34 (14.56)                         & 47.11 (13.07) \\ \cline{1-1}
\textbf{14}                   &                                         & 16.64 (15.17)                         & 25.73 (11.66) \\ \cline{1-1}
\textbf{2}                    &                                         & 24.14 (11.83)                         & \cellcolor[HTML]{D9D9D9}11.88 (16.8) \\ \cline{1-1}
\textbf{3}                    &                                         & 28.83 (8.86)                          & 38.36 (13.72) \\ \cline{1-1}
\textbf{5}                    &                                         & 30.43 (4.14)                          & 27.68 (4.5) \\ \cline{1-1}
\textbf{6}                    &                                         & \cellcolor[HTML]{D9D9D9}12.56 (13.11) & 28.12 (17.66) \\ \cline{1-1}
\textbf{8}                    &                                         & 28.39 (16.74)                         & 32.59 (7.49) \\ \cline{1-1}
\textbf{9}                  &                                         & 30.92 (9.79)                          & 45.28 (4.85) \\ \cline{1-1}
\textbf{P1-1}                 & \multirow{-10}{*}{\textbf{1}}           & 26.65 (17.48)                         & 32.07 (2.11) \\ \cline{1-4}
\multicolumn{2}{|c|}{\textbf{overall}}                         & 24.23 (13.24)           &  26.11 (16.21) \\ \cline{1-4}
\multicolumn{2}{|c|}{\textbf{total}}  &   \multicolumn{2}{c|}{25.21 (14.58)}   \\ \cline{1-4}
\end{tabular}}
 \label{tab:iaa}
\end{table}








==> table/subcategories.tex <==
\begin{table}[]
\begin{tabular}{l}
\hline
\textbf{Case fact} \\ \hline
\begin{tabular}[c]{@{}l@{}}whether is unanimously decided by \\ the court (unanimous)\end{tabular} \\ \hline
article violated or not (violated) \\ \hline
\begin{tabular}[c]{@{}l@{}}whether listed as keycase by \\ the court (keycase)\end{tabular} \\ \hline
\textbf{\begin{tabular}[c]{@{}l@{}}Legal Context: what type of allegation(s) \\ were raised under the specific articles\end{tabular}} \\ \hline
\begin{tabular}[c]{@{}l@{}}whether is the main alleged article \\ (proxy: allegation in the hudoc meta-data) (meta)\end{tabular} \\ \hline
allegated under which allegation (artX) \\ \hline
interpretate from procedural of substantive aspects \\ \hline
\textbf{Annotor's subjectivity} \\ \hline
different training/education background \\ \hline
different outcome prediction (pred\_diff) \\ \hline
\begin{tabular}[c]{@{}l@{}}different familiarity with the case/\\ whether know the case before (known\_diff)\end{tabular} \\ \hline
\end{tabular}

\caption{++++++++++ TODO categories need updates ++++++++++++ Subcategories of disagreement in legal explaination annotation in ECHR}
\label{tab:features}
\end{table}


==> text/RQ2.tex <==
We assess whether human-written case summaries, which act as proxy for explaining how the outcome of a case, can be helpful to derive the expert annotated relevance markup automatically. This approach has been inspired from \cite{prasad2021extent}, which used human-written explanations for Natural Language Inference data to derive expert annotations. %Unlike their work which deals with NLI task, where both the inputs (premise, hypothesis) along with explanations are of shorter length which fits within the input budget of BERT family models (512), we deal with longer input sequence of case facts and longer sequence of summary text (i.e explanations). In addition, The human-written summaries of the case judgement in ECHR’s public database HUDOC comprises of sections for facts and the law separately, in which they summarize the facts crucial to the case at hand and the reasoning behind the application of the convention articles to the case respectively. 
%We investigate  not only  both the the importance of with the facts section % alone in summary but also along with and the law section to derive relevance markups. 
We experiment with a `hard' and `soft' method to derive the relevance markup from summaries.%, namely (i) Hard method %which measures the direct word overlap between the input facts and summary explanation 
%and (ii) Soft method.
%which utilize summary-informed models to derive the relevance markup i.e models' takes explanation summary along with case facts as input to derive the outcome and we posit in this process, the model learns to interrelate the the summary explanations to the case facts to shift its focus to the relevance tokens in the input to arrive at the outcome prediction.

\subsection{Hard Method}
Our hard method derives a binary relevance markup using the direct overlap between stemmed words  in the case facts and summary explanation.\footnote{We used the SnowballStemmer from NLTK.}
% The human-written summary of the case judgement in ECHR’s public database HUDOC comprises of sections for facts and the law separately. 
The human-written summaries of case judgements in the public HUDOC database summarize the core facts in the case at hand and the reasoning behind the application of the convention articles to the case in separate `facts' and `law' sections. We parse the summary into these two sections using regular expressions. The law segment can be further decomposed to obtain the granularity of every article alleged to be violated. We use the facts along with specific article related law summary section to derive the binary relevance markup for that case-alleged article pair. \footnote{Note that not all the summaries have article-level sub-sections with respect to all allegations made. Where article-specific summary is not available, we only use the facts section of the summary as the proxy explanation corresponding to that article.} 
%Concretely, we define the hard method as follows: Given a case fact {x} and facts section of the summary concatenated with specifc article summary derived from the law section of the summary ${y_a}$ corresponding to article a, we obtain the binary relevance markup vector $H_{x,y,a}$ where the $i^\text{th}$ element is 1 if the stemmed word $x^\prime_{i} \in {y}^\prime$ and $x^\prime_{i}$ is not a stop word \footnote{We used the SnowballStemmer from NLTK \cite{bird2009natural}}; the i-th element of the vector is 0 otherwise, $x^\prime$ and $y^\prime$ denote the stems of the words $x_i$ and $y_i$ respectively\\
\iffalse
\begin{equation}
 H_{(x, y, a)} = [\text{ 1 if }  x^\prime_{i} \in y^\prime \text{ else 0 for } x^\prime_{i} \in x^\prime] 
\end{equation}
\fi
\subsection{Soft Method}
The above described hard method fails to capture 
%alternate variants of expressing the summary explanation text through 
paraphrases, synonyms, etc., when deriving a relevance markup for case facts. We experiment with remedying this problem by resorting to a `soft' method, in which we train models that take the case facts as input along with the summary as proxy for explanation and the alleged article information to predict the violation outcome. Then we derive the importance score of tokens using an explainability method, called `Integrated Gradients' \cite{sundararajan2017axiomatic} from explanation-informed model. We posit that the model learns to interrelate the the summary explanations to the case facts to shift its focus to the relevance tokens in the input to arrive at the outcome prediction.
%To make the model rely and learn the inter-relatedness between the provided explanation and the case facts, we also experiment with an additional auxiliary task where the model tries to predict the binary label indicating whether the given summary explanation is relevant to the case facts at hand.

\noindent \textbf{Base Architecture for Explanation-informed models}
\label{arch-rq2}
We reimplement and adapt the interaction model of \cite{santosh2023Zero} for the design of explanation-informed models. It is based on the Enhanced Sequential Inference Model by \cite{chen2017enhanced} to deal with long input sequences, following from hierarchical attention networks \cite{yang2016hierarchical}.
%It also incorporates conditional encoding  mechanism \cite{augenstein2016stance,rocktaschel2015reasoning} to learn the representation of case facts conditioned on the summary explanation. 
The model input consists of the case facts text $x$, the case summary $s$, and the set of articles alleged as a multi-hot vector $b$. Its output is to classify the set of articles $a$ that are deemed violated by the court. 
%We posit providing summary as an input and conditioning the case facts on the summary will aid the model to shift its focus on to more relevant tokens that are necessary to arrive at the violation prediction. 

%The input case facts description and the summary text are available at paragraph-level granularity from ECtHR. 
%But the length of each paragraph varies a lot and most of the times, observed to be less than 512 tokens (BERT token limit) which leads to padding them resulting in under utilization of resources for BERT computation. Hence 
We employ a greedy input packing strategy where we merge multiple paragraphs into one packet until it reaches the maximum of 512 tokens given by BERT models. If necessary, we break paragraphs across packets boundaries to fully use the text capacity.
%We do not truncate paragraphs abruptly if it exceeds the maximum length while packing, rather we form a new packet with the whole paragraph. 
%(As we observe in architecture model later, tokens in one packet do not interact directly with the tokens from other packet and thus abruptly truncating a paragraph during packing process will make it difficult for the model to capture the context of such truncated tokens from the previous packet.) 
%However if a single paragraph exceeds the maximum length, we truncate it to fit the packet maximum length (512) and fill the rest of the paragraph in the next packet.

%We obtain  $x = \{x_1, x_2, \ldots, x_m\}$ and $s = \{s_1, s_2, \ldots, s_k\}$ where $x_i = \{x_{i1}, x_{i2}, \ldots, x_{in}\}$ and $s_i = \{s_{i1}, s_{i2}, \ldots, s_{ip}\}$. ${x_i}$ (${s_i}$), ${x_{ij}}$ ($s_{ij}$), m (k) and n (p) denote $i^\text{th}$ packet, $j^\text{th}$ token in $i^\text{th}$ packet, number of packets, number of tokens in $i^\text{th}$ packet of the case facts description / case summary, respectively. $b$ and $a$ are provided in the form of $\{0, 1\}^p$ where p denoted  total number of modeled convention articles, 1 and 0 indicate a positive and negative  instance under allegation (violation) of that corresponding article in $b$ ($a$). 
Our explanation-informed model works as follows: We use pre-trained BERT models to obtain pre-interaction token encodings for each token in every packet, which are then aggregated to form packet representations using a token-level attention layer. A bidirectional GRU then contextualizes the packet representations. This procedure is done separately for the text of both facts and summaries. The interaction component then takes the dot product between packet representations of case facts and summary, thus making them both globally context-aware, similar to dot-product attention between questions and answers in QA-systems. We concatenate different combinations of pre-interaction and fact-aware packet representations of the summary through concatenation, difference and element-wise product, and vice-versa for the fact representation. We then merge both branches by conditioning the final representation of case facts on the final summary representation obtained through packet GRU and packet attention layer. This conditioning is done by initializing a bidirectional GRU layer's hidden state of the case facts branch with the post-interaction representation of the summary. This guides the GRU model to extract and refine the representations of case facts. We concatenate the obtained conditioned case facts representation with 
the multi-hot vector of allegation articles and use two fully connected layers to obtain the violation outcome. We calculate a binary cross-entropy loss over each article in the outcome vector. Figure \ref{fig:arch} (a) shows a schema of our used architecture.\footnote{For space reasons, the model description here is brief. We refer the interested reader to the code we will make publicly available upon publication.}
%captures interaction between the pre- and post-interaction representations
%using encoder for case facts and summary separately. 
%This layer takes the packet level representations of case facts $x$ and summary $s$ as input and outputs packet level representation of case facts and summary as $h = \{h_1, h_2, \ldots, h_m\}$ and $g = \{g_1, g_2, \ldots, g_k\}$ respectively.  We describe the encoding layer for case facts below in specific and same architecture is also used for summary. 
%We use a pre-trained BERT encoder to obtain token-level representations  $z_i = \{z_{i1}, z_{i2}, \ldots, z_{in}\}$ for packet ${x_i}$. Packet representations $f_i$ are computed via an attention mechanism as follows:
%where the most salient tokens in each packet are attended to. 
\begin{comment}
\begin{equation}
\scalemath{0.9}{
    u_{it} = \tanh(W_w z_{it} + b_w )  ~~\& ~~ 
    \alpha_{it} = \frac{\exp(u_{it}u_w)}{\sum_t \exp(u_{it}u_w)}  ~~\& ~~ 
    f_i = \sum_{t=1}^n \alpha_{it}z_{it}
\label{att}}
\end{equation}
\end{comment}
%where $W_w$,$b_w$ and $u_w$ are trainable parameters.
%and $\alpha_{it}$ represents the $t^\text{th}$ token-level importance in the $i^\text{th}$ packet. 

%$f= \{f_1, f_2, \ldots, f_m\}$, 
%capture the contextuality of all packets by 
%through a bi-directional GRU to obtain their context-aware version as $h = \{h_1, h_2, \ldots, h_m\}$. 
%Analogously, we obtain context-aware $g = \{g_1, g_2, \ldots, g_k\}$ for the summary.

%\noindent \textbf{Interaction:} This layer 
%captures the interaction between the packets of case facts description and summary explanations. First, we 
%takes the dot product between context-aware packet representations of case facts and summary. Then
%for each packet in the facts, 
%we compute the summary-aware representation and fact-aware representations based on relevant content from the packets: %using the weighted sum of  context-aware representations of summary packets according to the normalized dot product score. This process is represented 
\begin{comment}
\begin{equation}
\scalemath{0.9}{
    e_{ij} = h_i^Tg_j ~~\&~~  h_i^\prime = \sum_{j=1}^{k}\frac{\exp(e_{ij})}{\sum_{l=1}^{k}\exp(e_{il})} g_j ~~\&~~
g_j^\prime = \sum_{i=1}^{m}\frac{\exp(e_{ij})}{\sum_{l=1}^{m}\exp(e_{lj})} h_i}
\end{equation}
\end{comment}
%where $e_{ij}$ represents the %dot product 
%interaction score between the context-aware representations of $i^\text{th}$ packet of case facts and $j^\text{th}$ packet of case summary. $h_i^\prime$ and $g_j^\prime$ represents summary-aware representation corresponding to $i^\text{th}$ packet of case facts and fact-aware representation corresponding to $j^\text{th}$ packet of summary respectively. Thus we obtain  interaction-aware packet representations of the case facts and summary $h^\prime = \{h^\prime_1, h^\prime_2, \ldots, h^\prime_m\}$. and  $g^\prime = \{g^\prime_1, g^\prime_2, \ldots, g^\prime_k\}$

%\noindent \textbf{Post-interaction Encoding:}
%This layer utilizes the interaction-aware representations of both case-facts and summary to derive the final representation of case facts conditioned on case summary. Initially, 
%We first obtain the final summary representation and then use it to condition the final representation of case facts. We concatenate pre-interaction and fact-aware packet representations of the summary as follows:
\begin{comment}
\begin{equation}
    p_i = [g_i, g_i^\prime, g_i - g_i^\prime, g_i \odot g_i^\prime]
\label{eq_merge}
\end{equation}
\end{comment}
%where $\odot$ denotes the element-wise product.  This representation %through concatenation, difference and element-wise product intend to 
%captures interaction between the pre- and post-interaction representations. 
%representations of the packets in the summary 
%\cite{chen2017enhanced}. Then the final packet representations %$p = \{p_1, p_2, \ldots, p_k\}$ 
%are passed over a non-linear projection and a bi-directional GRU  to obtain the context-aware representations  $p^\prime = \{p^\prime_1, p^\prime_2, \ldots, p^\prime_k\}$ . Then all the packet representations are aggregated by an attention mechanism to obtain the final summary representation $S$ as described in Eq. \ref{att}. 
\iffalse
\begin{equation}
    u_{i} = \tanh(W_s p^\prime_{i} + b_s )  
     ~~\& ~~ 
    \beta_{i} = \frac{\exp(u_{i}u_s)}{\sum_i \exp(u_{i}u_s)}  ~~\& ~~ 
   S = \sum_{i=1}^k \beta_{i}p^\prime_{i}
\label{eq_sentatt}
\end{equation}
%where $W_s$,$b_s$ and $u_s$ are trainable parameters and $\beta_{i}$ marks the importance of $i^\text{th}$ packet in the summary.  
\fi
%Once we obtain the final summary representation $S$, we use that as a conditional encoding \cite{augenstein2016stance, rocktaschel2015reasoning} to obtain the final representation of case facts. 
%The final fact representations are computed analogously by combining the pre- and post-interaction representations, and then passing them through a non-linear projection and a bi-directional GRU. To condition them on the summary \cite{augenstein2016stance}
%,rocktaschel2015reasoning}
%, we initialize the GRU hidden state with the final representation of the given summary. This guides the GRU model to extract and refine the representations of case facts.
%not only based on the neighbouring packet contexts but also 
%Then all the packet representations are aggregated to obtain the final representation of case facts $C$ using the same attention computation described in Eq. \ref{att} .


%\noindent \textbf{Classification Layer:} %In this layer, 
%We concatenate the above obtained case facts representation $C$ with %the set of allegation articles by concatenating 
%the multi-hot vector $b$ of allegation articles 
%with the obtained case feature representation $C$ 
%and use a two fully connected layers to obtain the violation outcome. We calculate a binary cross-entropy loss over each article in the outcome vector. 
%as the violation outcome vector being a multi-hot vector.

\noindent \textbf{Auxiliary Task} We also add an auxiliary task along with the main violation outcome task in which the model is made to predict the binary label indicating whether the provided explanation is relevant to the current case facts or not.  
%The model trained for violation prediction task alone may learn to ignore the summary information and learn the violation prediction from case facts alone. However,
This ensures the model to 
%the main goal for this explanation-informed model is to 
learn the inter relatedness between the case facts and summary. % which finally result in shifting the models focus towards those tokens in the input case facts  that are relevant to arrive at the final violation outcome. In order to learn this dependency, 

\begin{figure*}[htp]
\caption{Base Model Architectures}
\centering
\begin{subfigure}[t]{.3\linewidth}
\caption{Explanation-informed model for soft match (RQ2)}
    \centering\includegraphics[width=\linewidth]{images/RQ2.png}
    
  \end{subfigure}
  \hfill
  \begin{subfigure}[t]{.3\linewidth} 
  \caption{Classification Variant for Legal Judgement Prediction (RQ3)}\centering\includegraphics[width=0.95\linewidth]{images/RQ3.png}
    
  \end{subfigure}
  \hfill
  \begin{subfigure}[t]{.3\linewidth}
  \caption{Article-aware prediction Variant for Legal Judgement Prediction (RQ3)}
\centering\includegraphics[width=0.85\linewidth]{images/RQ4.png}
    
  \end{subfigure}
\label{fig:arch}
\end{figure*}


\subsection{Dataset, Model Variants \& Metrics}
\label{rq2_dataset}

\noindent \textbf{Dataset}: ECtHR datsets created in previous works \cite{chalkidis2019neural, chalkidis2021paragraph, chalkidis2022lexglue, medvedeva2021automatic, aletras2016predicting} do not contain the summary texts, we create our dataset from scratch from a scrape of ECHR’s public database HUDOC. Note that the human summaries are not provided for all cases present in the database. We filter non-English cases based on the metadata. We extract the facts section from the judgement documents using regular expressions. Each case metadata contains the set of articles of the convention that were deemed violated by the court. We limit our set of articles to be the same 10 \cite{chalkidis2022lexglue}. We observed that the metadata present in HUDOC frequently did not correspond with the allegations mentioned in the judgment document, and hence we semi-manually curate allegation information for our text set. To obtain a corrected set of allegation articles, we first parse the conclusions section in the case judgement document. after noticing some alleged articles being mentioned in the texts were missing in the conclusion section, to improve quality, we also parsed section headers under the law section in the judgement. We did a manual inspection of all 50 sampled cases for annotation where allegations seemed to mismatch with, which amounted to about 25\% of cases. Our ECtHR experts consider this to be related to the way the court registry creates case metadata entries in HUDOC, which seems to lead to non-systematic inconsistences. While our test set has been manually curated, we leave an examination of this limitation of HUDOC metadata to future work. %\footnote{Note that the reasoning applied by the court with respect to each allegation is detailed in the law section of the judgement document.} document which mention the allegation about articles made by claimant. 

Again, the law section of the summary can be further parsed to obtain smaller summaries of every article allegation.
%i.e the court's reasoning to derive the violation outcome with respect to each alleged article is summarized in that section. We utilize the article-level granularity of law section in our hard method. When some articles don’t have summaries at article level, we use the whole law section as upper bound. 
We also notice that the law section of the summary mentions violation conclusions the court has reached with respect to every specific article alleged, and thus we remove that information present as the conclusion sub-section using regular expressions. Giving the conclusion section of the summary to the model would risk it learning this shortcut to derive the violation outcome directly rather than identifying legal reasoning in the explanation summary. While we utilize the article-level granularity of law section in the summary document for hard method, we  concatenate  all the articles summary in the law section for the soft method as the main task in soft method involves prediction of violation outcome for all articles under consideration.
% We leave the investigation of using only the specific article related law section in summary as the future work. 
We split the 2218 obtained case-summary pairs chronologically into training (1992-2016, 1718), validation (2017-18, 225) and test set (2019-2022/July, 275).
%The training, development and test sets  contain cases from  1992 - 2016, 2017 - 2018 and 2019 - 2022/July with 1718,225 and 275 respectively. 
% Detailed statistics about the dataset are presented in Table \ref{stat_rq2}. 
To experiment with the auxiliary task, we randomly sample two summaries per case from other instances in the training set to train the model predict the binary label corresponding to case fact-summary relevance.


\iffalse
\begin{table}
\centering

\caption{Dataset Statistics: number of words per case (\#Words/C), facts section of the summary (\#Words/S-F) and the summary (facts \& law section together) (\#Words/S )}
\scalebox{0.8}{
    \begin{tabular}{|p{1cm}|p{1cm}|p{1.5cm}|p{1.75cm}|p{1.5cm}|}
\hline
\textbf{Split} & \textbf{\#Cases} & \textbf{\#Words/C} & \textbf{\#Words/S-F} & \textbf{\#Words/S} \\ \hline
Train          & 1718             & 2810               & 196                  & 682                \\
Valid          & 225              & 3208               & 145                  & 800                \\
Test           & 278              & 3213               & 115                  & 970                \\ \hline
\end{tabular}}
  \label{stat_rq2}
\end{table}
\fi

\noindent \textbf{Models}
\label{model_rq2}
We experiment with three different pre-trained BERT encoders: plain BERT \cite{kenton2019bert}, LegalBERT \cite{chalkidis2020legal}, and CaseLawBERT \cite{zheng2021does}. While plain BERT is trained on general English corpora, the latter two are further pre-trained on English legal corpora. The LegalBERT pre-training corpora also consists of text from ECHR in addition to other corpus such as US, EU, UK legislation, contracts etc. 
%Court cases from European Court of Justice (ECJ) and European Court of Human Rights (ECHR) and US contracts. 
CaseLawBERT is pre-trained exclusively on legal decisions from US courts. 
We experiment with using
%to study of effect of adding law related section from the summary information additionally to the explanation: 
(i) only facts section of the summary (ii) Using facts and the law section of the summary, as well as with and without the auxiliary task.
%to study its effect.
These variants result in a total of 12 models shown in \ref{tab:rq2}. %reports the full resultsfollows: basemodel {X} $\in \{BERT, LegalBERT, CaseLawBERT\}$, section of summary used {Y}  $\in \{fact, fact+law\}$; and whether auxiliary task are added {Z} $\in \{aux, noAux\}$. 
%\subsubsection{Implementation Details} 
%We set token-level attention context vector, GRU dimension and packet-level attention context vector dimension in the pre-interaction encoding layer to be 300, 200 and 200 respectively. Classification layer for the main task and the auxiliary task have two layered networks with the hidden layer size set to be 200. The violation outcome classifier is trained with a binary cross entropy loss over each article and the auxiliary task classifier is trained with binary entropy loss over a one-hot vector. The model is optimized end-to-end using Adam \cite{kingma2014adam} optimizer. The dropout rate \cite{srivastava2014dropout} in all layers is 0.1.
We follow the hyperparameter settings as described in \cite{santosh2023Zero}.

\noindent \textbf{Evaluation Metrics}: \label{eval_RQ2} Our goal is to measure the alignment between the relevance markup derived automatically %(using explanation informed procedure from either hard match or soft match) 
and the expert annotation. For hard match, we obtain the token level importance scores as the output. While for soft match, we use Integrated Gradients (IG) \cite{sundararajan2017axiomatic} to obtain a focus score from the model at token-level with respect to the violation outcome of every alleged article in each case under consideration.  
%While the BERT family of models employ tokenizers which segment words into sub-word level, expert annotated relevance markups are at word level. Hence, 
We use max pooling over sub-words to obtain the word-level IG scores from the obtained sub-token level IG scores. %As these IG scores are on continuous scale, 
The continuous IG values were binarized using a threshold based on the density of annotations made by the annotator for each case-allegation-article pair. 
%For every alleged article under each case, we evaluate the Cohen's kappa coefficient \cite{cohen1960coefficient} $\kappa$ between the explanation derived importance scores and the experts' annotated relevance markup at token-level with removal of stop words.  
We report the overall agreement for each of the annotators as the average across Cohen's kappa \cite{cohen1960coefficient} $\kappa$ computed between the explanation derived importance scores and the experts' annotated relevance markup with removal of stop words for every case-allegation article pair under evaluation. 
%We also report  coefficient scores averaged per article considering only the cases in what that article is alleged.  We also report the  coefficient scores averaged per article separately under two heads - one in which we consider only the cases in which corresponding article is alleged by the claimant but not deemed violated by the court and the other in which we consider only cases in which article is both alleged and deemed violated by the court. 

In addition to alignment, we also report prediction performance on the test set. Following \cite{chalkidis2022lexglue}, we report micro-F1 (micF1) and macro-F1 (macF1) scores for 10+1 classes where 10 classes correspond to %violation outcome for 
10 articles under consideration and an additional label is created during evaluation 
%\footnote{Note that this additional label is only created during evaluation and we use 10 classes classifier for training.} 
corresponding to a non-violation of all 10 articles. 
%(i.e all 10 articles under consideration are not violated) and with label negative otherwise, in both target vector and predictions. 
Following \cite{santosh2022deconfounding}, we also report hard-macro-f1 (hm-F1), which is the mean F1-score computed for each article computed with negative instances restricted to those cases in which an article has been alleged but not deemed to have been violated. 
%We believe this to be an important measure in our setting of Task A|B as in the metrics of  micro-F1 ($\mu$-F1) and macro-F1 (m-F1), the cases in which a particular article has been deemed violated is considered as positive but the rest of the instances are considered negative. Among the rest which are deemed to be non-violation, there are two categories of cases, one in which article is not even alleged and the other being in which article is alleged by the claimant and court decided to be of non-violation. While the former category can be simply learnt from the allegation information which we are providing as input to the model, the latter is of utmost critical as it requires the model to reason about the factors that lead to the violation. 

%Further to understand the effect of how much model has learnt to inter relate the explanations and  case facts, we also create models which do not use summary as input but only takes input case facts and alleged articles and predicts the violation outcome. We derive these models without the interaction and post interaction components (This is similar to the architecture in RQ3). The prediction performance difference between this model and the explanation-informed models validates our hypothesis that providing explanation as an additional input helps the model to shift their focus to actual relevant words in arriving at the prediction outcome.


\subsection{Discussion \& Analysis}
%The aim of RQ2 is to assess the feasibility of using human-written case summaries for automatically deriving expert-annotated rationales. We experiment with two methods: (i) the Hard method which measures the direct word overlapping, and (ii) the Soft Method, which leverages summary-informed models to derive the relevance markup. 
We report the performance of our soft and hard method along with a random baseline for RQ2 in Table \ref{tab:rq2}. 
Overall, our proposed methods score higher than the random baseline in alignment with both annotators, indicating the principle utility of deriving these markups using an explanation-informed way. In general, model alignment with annotator 1 is higher than with annotator 2. This is in part due to a difference in density of markups, as annotator 1 has a relatively higher density of marked up tokens (11.2\% on average compared to the annotator 2 with a density of 9.3\%). Surprisingly, we notice a higher agreement score in the hard method compared to the soft method. We conjecture that the simple overlap based method being effective due to (i) the nature of human-written summaries available from HUDOC which tend to contain wording very close to the case with little paraphrasing and (ii) our fine-grained hard method design in which we extract the article-level sub-section in the law section of summary leading to high overlap of terms at the article-level relevance markups. While in soft method, we merge all article summaries in the law section along with facts as a summary input, as the primary task used there is to predict the violation outcome for all the articles under consideration. A possible future experiment could be to only use the specific article related law sub-section in the summary and modifying the primary task to deal with a specific article only.

Among the soft methods, our hypothesis of adding an auxiliary task results in an overall improvement in violation prediction task allowing the model to learn the inter-relatedness between the facts and the summary. But this did not translate into an improvement in the alignment performance. Analogously, on the other hand, adding law section along with facts in the summary resulted in a marginal drop in performance with no substantial change in the alignment performance. More surprisingly, neither law-specific domain related pre-training in CaseLawBERT nor the ECHR corpus related pre-training in LegalBERT did not help for improving the alignment performance. The overall similar performance among the variants of soft method and its under performance to hard method can likely be attributed to these neural models falling prey to various distracting spurious correlations that exist prominently in the ECtHR judgements dataset, that suffer from fact statements not being finalized until the case outcome is known leading to such confounding effects as demonstrated in \cite{santosh2022deconfounding}. %Despite this limitation, we believe this explanation informed setup can motivate the community in development of robust legal NLP models that learn to interrelate case facts and summary text in a way that results to better alignment performance. 



==> text/RQ4.tex <==
Previous approaches \cite{aletras2016predicting, chalkidis2019neural, chalkidis2021paragraph,chalkidis2022lexglue, medvedeva2020using, medvedeva2021automatic, santosh2022deconfounding} involved with Legal Judgement Prediction tackled it as a classification problem (as we have dealt in RQ3) which takes the case fact alone as the input.  This way of formulation neglects the role of underlying legal sources which are used to deduce the outcome, unlike how the legal practitioners identify the relevant rules from legal sources and apply them to analyze the case at hand. Recently, \textbf{cite our entailment} have proposed to tackle this task as an entailment approach where they provide the model with the input as pairs of case fact description along with candidate ECHR articles and predict a binary target label determining the violation of provided candidate article. They  posit that the classification paradigm may lead the model to learn the statistical correlations that exist between the decision outcome and textual features which may not be legally relevant. This effect is also demonstrated in the work by Santosh et al. \cite{santosh2022deconfounding} where models fall prey to distractor tokens learning spurious shortcuts rather than actual tokens causally related to arrive at the outcome.  Though, they  hypothesized that this entailment setup can help the model to overcome the spurious shortcut problem, they did not explicitly measure the improvement in models' alignment with experts annotation. In this work, we bridge that gap by assessing the entailment models from an alignment perspective. 

We describe the entailment task and the model base architecture for Legal Judgement Prediction in subsection \ref{arch_rq4}. Then we describe the dataset, model variants and the metrics in subsection \ref{dataset_rq4} and finally report our results and observations in subsection \ref{disc_rq4}. 

\subsection{Task \& Base Model Architecture}
\label{arch_rq4}
Entailment variant for Task A|B is defined as follows:  Given the case fact textual description along with a particular article information in addition to the allegation information of that article by the claimant, the model should predict the binary outcome whether the given article has been violated or not by the court.

We use the entailment architecture for LJP from \textbf{cite our entailment} which is also described in our Soft method in Section \ref{arch-rq2}. The main differences between the entailment architecture from the soft method architecture is as follows: (i) In place of explanation, we take article text as input. As article text is not very long, we do not apply greedy packing strategy to article text. (ii) The allegation information, we provide here $b$ only corresponds to the article in the input rather than all the articles as in soft method. Hence, we use a single binary value rather than multi-hot vector.  (iii) Output classification layer will be a binary variable indicating the violation of that article rather than multi-hot vector of violations of all the articles. 

\subsection{Dataset, Models \& Evaluation Metrics}
\label{dataset_rq4}
\subsubsection{Dataset} Following \textbf{our entailment}, we use the LexGLUE benchmark ECtHR Task and Task B dataset as similar to our RQ3.They augment the dataset with the texts of the 10 articles in the label set from the publicly available ECHR convention document\footnote{https://www.echr.coe.int/documents/convention\_eng.pdf}. We follow the same splits for training, validation and test.

\subsubsection{Models} We create three variants of entailment model by using different pre-trained BERT encoders such as BERT \cite{kenton2019bert}, LegalBERT \cite{chalkidis2020legal}, CaseLawBERT \cite{zheng2021does}. 

\subsubsection{Evaluation Metrics} 



\subsection{Discussion \& Analysis}
\label{disc_rq4}

==> text/anno_guidance.tex <==
%In a paper co-authored by lawyers, we must start out with a definition of what “annotation” here means. 
For purposes of our work `annotation' means the highlighting of words and parts of sentences in fact sections of judgements and decisions of the ECtHR which experts deemed relevant for the legal evaluation of whether the text supports a violation of the rights contained in the ECHR.  The aim of our double annotation (i.e., an annotation of the same fact pattern by two experts) is to study to what degree ECHR legal experts agree on what elements of the facts are relevant for the violations of which articles. `Agreement' here refers to a mathematical measure of the overlap of annotated text spans between the experts. It does not refer to any violation prediction by the experts. %The further aim was to develop machine learning models that, given a case fact description, can identify text segments that contain factual information relevant for the determination about whether a given article has been violated.
We developed annotation guidelines to facilitate congruence in our approach. A set of initial instructions were tested with 10 cases in a trial phase, after which the final guidelines were completed. The full guidelines will be published along with dataset. The following serves as a short summary:

Annotators were given the fact statements excerpted from ECtHR judgments along with information about which articles had been alleged to be violated. They were asked to annotate, for each article, relevant text segments. “Relevant” in this context meant that highlighted parts of the texts, in the eyes of a human lawyer, would be important to assess whether a certain fact pattern gives rise to a violation of the convention. Put differently, this means marking up text segments reflecting specific facts that increase the likelihood of the Court reaching the conclusion that a certain Convention article has been violated or not, respectively.
%Typically this is because the fact in question relates to a requirement of a legal rule that is either part of the Convention, the law as developed in ECtHR’s jurisprudence. 
%We were instructed by our co-authors on the technical side not to try to guess the perspective of an algorithm “learning”, but to stay in the realm of our “human” expertise. So, in short, we were looking for text segments reflecting specific facts that increase the likelihood of the Court reaching the conclusion that a certain Convention article has been violated or not, respectively.

%By relevant we also tried to include the pertinent context for a violation. For example, in freedom of speech cases, the incriminated speech needs to be assessed against the context of a case, the history of a given country (eg Nazism in Germany).; in other words, it is the specific composition of facts in their context that we aimed to reflect in the annotation.

%We did not annotate spurious or redundant facts, i.e., words, phrases or facts that were not relevant to a finding regarding the presence or absence of a violation.

Text should be annotated at token span level (e.g. three consecutive words) and not whole sentences unless all of their content was deemed relevant. %We did so by clicking and dragging the mouse cursor as you would in a regular text processing environment. Once the cursor was released, a drop-down menu with the available types appeared to select from the various articles and possible violations. We started and ended at the word level. Punctuation was not relevant, especially not brackets, which, however, often indicate a specific meaning given to a word or text segment, or transport a certain highlight the Court attaches to an expression. 
Typically annotated segments contained specific fact patterns; single- or multiword expressions indicating relevant legal concepts; mentions of domestic laws or regulations; specific sequences of events that have a bearing on the finding of a violation or that could justify discarding the applicant’s allegation of violation. While the facts statements occasionally contained information about domestic law or domestic jurisprudence, only such aspects that the ECtHR would directly take into account were to be annotated. Other specific elements of the instructions included the treatment of dates and events, time spans, and repetitive/enumerative statements of fact patterns. All annotation was done in the GLOSS annotation tool.

%Where the Strasbourg Court relied extensively on domestic courts’ decisions or law, we annotated facts that were relevant for the alleged violation and not general statements regarding the interpretation of domestic law, even if the interpretation was made in light of the Convention. This was avoided in order to not distort the data with the interpretation of other Courts. We were specifically looking for facts that would be taken into account in the proportionality assessment of the Court, that is, the “weighing material” of the national court decision was relevant - even if the legal evaluation of that material differs from the national court.

%We annotated specific dates only in cases where those dates disclose events that are relevant for the assessment of the substance of the article, eg where the arrest is supposed to happen only for a limited time (24 hours or 3 days) or for example length of procedure cases.

%We were provided with an annotation environment (gloss), and were given the facts of the cases, which were drawn from HUDOC. 
It is important to underline that ECtHR fact descriptions are not objective accounts of facts. They have been trimmed by the Registry of the Court and do not represent the applicant’s original allegations. There has also been an exchange between the government and the applicant, and thus the final version is drafted after those facts have been ‘set straight’. Also, the Court itself does usually not engage in fact-finding but relies on the account of facts given to it by the parties; the quality and the quantity of facts from the national proceedings vary greatly.% It is usually a lawyer from the registry from the respective respondent country who drafts the facts of a case. 
Also, the Court has sought over the past years, to streamline the process of finalizing judgments \cite{villiger2022handbook} %\footnote{Mark Villiger, Judgment: European Court of Human Rights (ECtHR) in Max Planck Encyclopedia of International Law, online, December 2017, para 23}
All of this explains why the sets of facts to be found on HUDOC vary considerably as to their richness of detail, length and general structure, as well as level of abstraction. Nevertheless, our working hypothesis was that the facts are drafted by the Court in a manner that best suits the finding or non-finding of a violation. %It is interesting to see that sometimes, the Court provides headlines in the facts that contain a evaluation (e.g. access to data in the Augsburg case).


%With judgments, the Court decides on the merits of a case, while decisions refer to admissibility decisions, that is, decisions where the Court usually dismisses a case at an early stage of the proceedings, without finding a violation. We excluded friendly settlements. (time frame of judgments of decisions – is that mentioned somewhere in the paper?). 

While experts were provided with information about which articles had been alleged, they did not know whether procedural or substantive aspects (negative or positive dimension of violations) of a norm were alleged to have been violated. If a segment of text was relevant for multiple alleged articles, it was annotated multiple times with types corresponding to those individual articles.%It should be noted that, in line with prior work, we only conducted annotations for the 10 ECHR articles that were part of the LexGLUE benchmark.

%Our co-authors instructed us annotators with the information of what articles (one or several) were alleged to have been violated in a given set of facts. In the first ten cases, the instructions were reliant on the metadata that HUDOC, the Court’s database, provides in the section “case details”; there, the Court provides for example information on which Articles were implicated in the judgment or decision. However, in view of the incongruence we discovered, that is, that the metadata did not correspond with the allegations in the actual decision or judgment, the other 40 cases were checked by our co-authors in order to ensure that the judgment or decision actually dealt with the allegations we were instructed to look for. 
%We did not, however, get details about the way the allegation of a given violation was laid out; in other words, we did not know whether procedural or substantive aspects (negative or positive dimension of violations) of a norm were alleged to have been violated. (I would think that more details here would give higher precision in the annotation – so eg if annotators knew the whole sentence where the Court describes what the applicant alleges; this is very important in cases where multiple violations were alleged; however, I am also quite afraid that this is not really something that can be automated very well?)

%In case of conjoint articles (for example Articles 8 and 14, 13 and 8) and in cases where the alleged violations are reflected in the same set of facts (e.g. the right to privacy and the right to be free from inhumane treatment, the right to property and the prohibition of discrimination) given that the Court might decide for instance that the fact give rise to a violation under the procedural aspect of Article 8 and ignore Article 13 we annotated the same set of facts with the different colours, representing the different violations for the two articles. 

%We had previously agreed to only annotate Articles 2 to 11, right to property in Article 1, Protocol 1; we did also annotate Article 14 ECHR, the prohibition of discrimination, which is a right that does not have an independent scope of application, but always depends on another substantive right. We excluded Article 13 ECHR as well as all other substantive rights in additional protocols, such as the right to vote and the right to education. 
%Via a tool, we could use colored markings for each article; that is, for example all words that we found relevant for a violation of Article 9, the freedom of religion, were marked in the color purple. It was also possible to mark words or sets of words in two or more different colors, that is, marking them as relevant for more than one violation, eg Article 9 ECHR, the freedom of religion and at the same time, Article 14 ECHR, the prohibition of discrimination. 

%We tried to differentiate repetitive phases in our annotations. The underlying rationale is to flesh out only relevant factual patterns and avoid unnecessary and rhetorical language.
%A repetitive phrase occurs when the same fact pattern is written about multiple times in the text. This mainly happens for three reasons, each of which lead to different treatment during annotation:
%\begin{itemize}
%    \item 	To illustrate the regularity of some event, where one such event would suffice for the legal assessment. In such cases, only one example mention needs to be annotated. We are only looking for facts which reveal the domestic authorities’ diligence in dealing with the applicant’s allegation (typically the one mentioned first)
%Example: Cases of prolonged detention in which domestic courts only repeat the initial reasons for arrest without reasessing the applicant’s situation
%\item Because the presence of repetitiveness is legally decisive, in which case all instances are to be annotated
%\item If a fact pattern changes over time or is presented in contradictory perspectives (e.g., differing diagnosis of a mental illness) AND the diversity of information/views will be decisive for the court’s assessment (e.g., in determining discharge of positive obligations by the respondent state), then all instances should be annotated.


%One of the reasons we embarked into this project was the hope to make a contribution to the identification of the causes of judicial inconsistencies in the ECHR’s case law.  

%Both annotators operated under the assumption that the Court does deploy one single legal yardstick when analysing facts and deciding, based on those facts on the substantive provisions of the application. There are currently 46 States Signatories of the Convention (now that Russia has left the Council of Europe) and according to the subsidiary doctrine/margin of appreciation which is the cornerstone of the Convention, when deciding upon a case, the Court defers to the initial assessment of the domestic authorities). Given such specific architecture, it is unrealistic to believe that the Court uses the same 'metric to analyse 46 different domestic systems. However, given that the literature on the ECHR is replete with various explanations of this phenomenon \cite{spano2018future} we decided to change the perspective upon the issue of inconsistencies and take a step-back into previous phase of legal argument drafting and focus on how facts are qualified by the Court as being relevant for a provision or not.
